Distributed Random Reshuffling over Networks

In this paper, we consider distributed optimization problems where $n$ agents, each possessing a local cost function, collaboratively minimize the average of the local cost functions over a connected network. To solve the problem, we propose a distributed random reshuffling (D-RR) algorithm that invokes the random reshuffling (RR) update in each agent. We show that D-RR inherits favorable characteristics of RR for both smooth strongly convex and smooth nonconvex objective functions. In particular, for smooth strongly convex objective functions, D-RR achieves $\mathcal{O}(1/T^2)$ rate of convergence (where $T$ counts epoch number) in terms of the squared distance between the iterate and the global minimizer. When the objective function is assumed to be smooth nonconvex, we show that D-RR drives the squared norm of gradient to $0$ at a rate of $\mathcal{O}(1/T^{2/3})$. These convergence results match those of centralized RR (up to constant factors) and outperform the distributed stochastic gradient descent (DSGD) algorithm if we run a relatively large number of epochs. Finally, we conduct a set of numerical experiments to illustrate the efficiency of the proposed D-RR method on both strongly convex and nonconvex distributed optimization problems.

==> DRR_TSP Final/supplementary_R1.tex <==
\section*{Supplementary Material}

\setcounter{section}{1}
\section{Parts of Proofs for strongly convex case}

\subsection{Proof of Lemma \ref{lem:rhow}} 
\label{app:lem_rhow}
\begin{proof}
    Based on Assumption \ref{ass:W}, we have 
    \begin{align*}
        \norm{W\bs{\omega} - \1\bar{\omega}^{\T}} &= \norm{\prt{W-\frac{1}{n}\1\1^{\T}}\prt{\bs{\omega} - \1\bar{\omega}^{\T}}}\\
        &\leq\norm{W - \frac{1}{n}\1\1^{\T}}\norm{(I - \frac{1}{n}\1\1^{\T})\bs{\omega}}.
    \end{align*}
\end{proof}

\subsection{Proof of Lemma \ref{lem:sigma}}
\label{app:lem_sigma}
\begin{proof}
     {Using \eqref{eq:muL} and \eqref{eq:limit_avg}, it follows}
    \begin{align}
        %&\quad \E\brk{\frac{1}{n}\sumn \fp{i}{\ell}(\bxs{\ell}) - \frac{1}{n}\sumn \fp{i}{\ell}(x^*) - \inpro{\frac{1}{n}\sumn\nabla \fp{i}{\ell}(x^*), \bxs{\ell} - x^*}}\nonumber\\
        & \E\brkn{D_{\bar{s}_\ell}(\bxs{\ell}, x^*)}
        \leq \frac{L}{2}\E\brkn{\normn{\bxs{\ell} - x^*}^2}\nonumber\\
        &= \frac{L {\alpha_t^2}}{2}\E\brk{\norm{\sum_{k=0}^{\ell - 1}\prt{\frac{1}{n}\sumn \nabla \fp{i}{k}(x^*)}}^2}\nonumber\\
        &\leq \frac{L {\alpha_t^2}}{2n}\sumn \E\brk{\norm{\sum_{k=0}^{\ell - 1}\nabla\fp{i}{k}(x^*)}^2} \nonumber\\
        &=  {\frac{L{\alpha_t^2}}{2n}
        \sumn\frac{\ell(m-\ell)}{(m-1)m}\sum_{j=1}^{m}\normn{\nabla f_{i,j}(x^*)}^2} \leq \frac{L\alpha_t^2 m}{4}\sigma_*^2\label{eq:sigma_s2},
    \end{align}
    where %\eqref{eq:sigma_s1} holds for convexity of norm and 
    \eqref{eq:sigma_s2} holds according to Proposition 1 in \cite{mishchenko2020random}. The lower bound can be derived similarly.
\end{proof}

% \subsection{Proof of Lemma \ref{lem:lya}}
% \label{app:lem_lya}
% \begin{proof}
%     \textbf{Step 1: Obtain a combined recursion $H_t^{\ell}$}.
%     Combining Lemmas \ref{lem:xbar0} and \ref{lem:cons0}, we obtain
%     \begin{align}
%         &H_t^{\ell + 1} \leq \brk{\prt{1-\frac{\alpha_t\mu}{2}} + \frac{30n\alpha_t^2 L^2}{1-\rho_w^2}\omega_t}\E\brk{\norm{\bx{t}{\ell} - \bxs{\ell}}^2}\nonumber\\
%         &\quad + \brk{\frac{2\alpha_t L^2}{n}\prt{\frac{1}{\mu} + \alpha_t} + \frac{1+\rho_w^2}{2}\omega_t}\E\brk{\norm{\x_t^{\ell} - \Bxt{\ell}}^2}\nonumber\\
%         &\quad + 2\alpha_t\svar\prt{1 + \frac{15\alpha_tnL\rho_w^2}{1-\rho_w^2}\omega_t} + \frac{15n\rho_w^2\alpha_t^2\sigma_*^2}{1-\rho_w^2}\omega_t\label{eq:At_s1}
%     \end{align}
    
%     $\omega_t$ is chosen so that the following inequalities hold for all $t, \ell$, 
%     \begin{subequations}
%         \label{eq:wt_in}
%         \begin{align}
%             &\quad \prt{1-\frac{\alpha_t\mu}{2}} + \frac{30n\alpha_t^2 L^2}{1-\rho_w^2}\omega_t \leq 1 - \frac{\alpha_t\mu}{4}\label{eq:wt1}\\
%             &\quad \frac{2\alpha_t L^2}{n}\prt{\frac{1}{\mu} + \alpha_t} + \frac{1+\rho_w^2}{2}\omega_t \leq \prt{1 - \frac{\alpha_t\mu}{4}}\omega_t\label{eq:wt2}
%         \end{align}
%     \end{subequations}
    
%     We verify the choice of $\omega_t$ in \eqref{eq:wt}. Firstly, \eqref{eq:wt2} is equivalent to 
%     \begin{equation}
%         \label{eq:wt2_s1}
%         \prt{\frac{1-\rho_w^2}{2} - \frac{\alpha_t\mu}{4}}\omega_t \geq \frac{2\alpha_t L^2}{n}\prt{\frac{1}{\mu} + \alpha_t}.
%     \end{equation} 
    
%     Noting $\alpha_t \leq \frac{1-\rho_w^2}{{   2}\mu}\leq \frac{1}{\mu}$, we have 
%     \begin{align*}
%         &\frac{1-\rho_w^2}{2} - \frac{\alpha_t\mu}{4} \geq \frac{1-\rho_w^2}{2} - \frac{1-\rho_w^2}{8} = \frac{3(1-\rho_w^2)}{8}, \\
%         &\frac{2\alpha_t L^2}{n}\prt{\frac{1}{\mu} + \alpha_t} \leq \frac{4\alpha_t L^2}{n\mu}.
%     \end{align*}
    
%     Thus, it is sufficient for $\omega_t \geq \frac{16\alpha_t L^2}{n\mu(1-\rho_w^2)}$ to satisfy \eqref{eq:wt2_s1}. 
    
%     Secondly, \eqref{eq:wt1} requires $\omega_t \leq \frac{(1-\rho_w^2)\mu}{120n L^2}\frac{1}{\alpha_t}$ or $\frac{16\alpha_t L^2}{n\mu(1-\rho_w^2)}\leq \frac{(1-\rho_w^2)\mu}{120n L^2}\frac{1}{\alpha_t}.$ It is sufficient that $\alpha_t \leq \frac{(1-\rho_w^2)\mu}{8\sqrt{30} L^2}$. We thus obtain a recursion for $H_t^{\ell}$ according to \eqref{eq:wt_in} and \eqref{eq:At_s1}: 
%     \begin{equation}
%         \label{eq:At_ell}
%         \begin{aligned}
%             H_t^{\ell + 1} &\leq \prt{1 - \frac{\alpha_t \mu}{4}} H_t^{\ell} + 2\alpha_t\svar\prt{1 + \frac{240\alpha_t^2\rho_w^2L^3}{\mu(1-\rho_w^2)^2}}\\
%             & + \frac{240\alpha_t^3\rho_w^2 L^2}{\mu (1-\rho_w^2)^2}\sigma_*^2
%         \end{aligned}
%     \end{equation}
    
%     \textbf{Step 2: Relate $H_t^{\ell}$ with the outer loop.} 
%     Unroll \eqref{eq:At_ell} with respect to $\ell$ and notice $\alpha_t$ is unchanged for $\ell \geq 0$, we obtain, 
%     \begin{align}
%         \label{eq:Atm}
%         H_t^m &\leq \prt{1 - \frac{\alpha_t\mu}{4}}^m H_t^0 + 2\brk{\alpha_t\svar\prt{1 + \frac{240\alpha_t^2\rho_w^2L^3}{\mu(1-\rho_w^2)^2}} \right.\nonumber\\
%         &\left. + \frac{120\alpha_t^3\rho_w^2 L^2}{\mu (1-\rho_w^2)^2}\sigma_*^2}\brk{\sum_{k=0}^{m - 1}\prt{1 - \frac{\alpha_t\mu}{4}}^k}.
%     \end{align}
    
%     Note from Algorithm \ref{alg:DGD-RR} and \eqref{eq:limit_avg}, we have the following facts:
%     \begin{equation*}
%         x_{i,t}^m = x_{i, t+1},\quad x_{i,t}^0 = x_{i,t} = x_{i, t - 1}^m, \quad \bxs{0} = x^* = \bxs{m}.
%     \end{equation*}
    
%     Therefore, 
%     \begin{equation}
%         \label{eq:in_out}
%         \begin{aligned}
%             &\quad \bx{t}{m} - \bxs{m} = \bar{x}_{t + 1} - x^*, \quad \bx{t}{0} - \bxs{0} = \bar{x}_t - x^*,\\
%             &\quad \x_t^m - \Bxt{m} = \x_{t + 1} - \1\bar{x}_{t + 1}^{\T},\\
%             & \x_t^0 - \Bxt{0} = \x_t - \1\bar{x}_t^{\T}.
%         \end{aligned}
%     \end{equation}
    
%     We then use $H_{t + 1}$ to denote $H_t^{m}, \forall t\geq 0$, i.e., 
%     \begin{align}
%         \label{eq:At_outer}
%         & H_{t+1} := \E\brk{\norm{\bar{x}_t^m - x^*}^2} + \omega_t \E\brk{\norm{\x_t^m - \Bxt{m}}^2}\nonumber\\
%         &= \E\brk{\norm{\bar{x}_{t + 1} - x^*}^2} + \omega_t \E\brk{\norm{\x_{t + 1} - \1\bar{x}_{t + 1}^{\T}}^2}.
%     \end{align}
    
%     Substitute $H_t$ into \eqref{eq:Atm}, we obtain the recursion for the outer loop $t$ : 
%     \begin{align*}
%         H_{t + 1} &\leq \prt{1 - \frac{\alpha_t\mu}{4}}^m H_t + 2\brk{\alpha_t\svar\prt{1 + \frac{240\alpha_t^2\rho_w^2L^3}{\mu(1-\rho_w^2)^2}}\right.\\
%         &\left. + \frac{120\alpha_t^3\rho_w^2 L^2}{\mu (1-\rho_w^2)^2}\sigma_*^2}\brk{\sum_{k=0}^{m - 1}\prt{1 - \frac{\alpha_t\mu}{4}}^k}.
%     \end{align*}
    
%     \textbf{A uniform bound for $H_t^{\ell}, \forall \ell.$} \eqref{eq:Atm} in Step 2 gives a uniform bound for $H_t^{\ell},\forall \ell$, 
%     \begin{align*}
%         H_t^{\ell} &\leq \prt{1 - \frac{\alpha_t\mu}{4}}^{\ell} H_t^0 + 2\brk{\alpha_t\svar\prt{1 + \frac{240\alpha_t^2\rho_w^2L^3}{\mu(1-\rho_w^2)^2}} \right.\\
%         &\left. + \frac{120\alpha_t^3\rho_w^2 L^2}{\mu (1-\rho_w^2)^2}\sigma_*^2}\brk{\sum_{k=0}^{\ell - 1}\prt{1 - \frac{\alpha_t\mu}{4}}^k}.
%     \end{align*}
% \end{proof}

\subsection{Proof of Lemma \ref{lem:At_ds}}
\label{app:lem_At_ds}
\begin{proof}
    Unroll \eqref{eq:At} in Lemma \ref{lem:lya} and invoke the relation between $\svar$ and $\sigma_*^2$ according to Lemma \ref{lem:sigma}, we get 
    \small
    \begin{align}
        & H_t \leq \prod_{j=0}^{t-1}\prt{1 - \frac{\alpha_j\mu}{4}}^m H_0 + \sigma_*^2\sum_{j=0}^{t-1}\crk{\brk{\prod_{q = j+1}^{t-1} \prt{1 - \frac{\alpha_q\mu}{4}}^m} \alpha_j^3\nonumber\right.\\ 
        &\left.  \brk{\sum_{k=0}^{m-1}\prt{1 - \frac{\alpha_j\mu}{4}}^k}
        \brk{\frac{Lm}{2} \prt{1 + \frac{240\alpha_j^2\rho_w^2L^3}{\mu(1-\rho_w^2)^2}} + \frac{240\rho_w^2L^2}{\mu(1 - \rho_w^2)^2}} }\nonumber\\
        &\leq \prod_{j=0}^{t-1}\prt{1 - \frac{\alpha_j\mu}{4}}^m H_0 + \sum_{j=0}^{t-1}\crk{\brk{\prod_{q = j+1}^{t-1} \prt{1 - \frac{\alpha_q\mu}{4}}^m} \alpha_j^3\nonumber\right.\\ 
        &\left.\brk{\sum_{k=0}^{m-1}\prt{1 - \frac{\alpha_j\mu}{4}}^k}}\prt{mL + \frac{240\rho_w^2L^2}{\mu(1 - \rho_w^2)^2}} \sigma_*^2\label{eq:At0}
    \end{align}\normalsize
    
    The last inequality holds for $\alpha_j^2 \leq \frac{(1-\rho_w^2)^2\mu}{240\rho_w^2 L^3}$ which is necessary for $\alpha_j\leq \frac{(1-\rho_w^2)\mu}{8\sqrt{30} L^2}$. {\kh Let $\alpha_t = \alpha$ in \eqref{eq:At0}. We obtain 
	\small
	\begin{equation}
		\label{eq:Ht_contant}
		\begin{aligned}
			& H_t \leq \prt{1 - \frac{\alpha\mu}{4}}^{mt} H_0 + \sum_{j=0}^{t-1}\crk{\brk{\prt{1 - \frac{\alpha\mu}{4}}^{m(t - 1-j)}}\right.\\
			&\left. \alpha^3\brk{\sum_{k=0}^{m-1}\prt{1 - \frac{\alpha\mu}{4}}^k}}
			\prt{mL + \frac{240\rho_w^2L^2}{\mu(1 - \rho_w^2)^2}} \sigma_*^2\\
			&= \prt{1 - \frac{\alpha\mu}{4}}^{mt} H_0\\
			& + \sum_{j=0}^{t-1}\sum_{k=0}^{m-1}\brk{\prt{1 - \frac{\alpha\mu}{4}}^{m(t - 1-j)+k}\alpha^3}\prt{mL + \frac{240\rho_w^2L^2}{\mu(1 - \rho_w^2)^2}} \sigma_*^2\\
			&\leq \prt{1 - \frac{\alpha\mu}{4}}^{mt} H_0 + \frac{4\alpha^2}{\mu} \prt{mL + \frac{240\rho_w^2L^2}{\mu(1 - \rho_w^2)^2}} \sigma_*^2.
		\end{aligned}
	\end{equation}\normalsize
	}
	Substitute $\alpha_t = \frac{\theta}{{    m}\mu(t +K)}$ into \eqref{eq:At0}, we obtain
    \small
    \begin{align}
        & H_t \leq \prod_{j=0}^{t-1}\prt{1 - \frac{\theta}{4{    m}(j + K)}}^m H_0\nonumber\\
        & + \sum_{j=0}^{t - 1}\crk{\brk{\prod_{q = j + 1}^{t - 1}\prt{1 - \frac{\theta}{4{    m}(q + K)}}^m} \frac{1}{(j + K)^3}\nonumber\right.\\
        &\quad\left. \brk{\sum_{k=0}^{m - 1}\prt{1 - \frac{\theta}{4{    m}(j + K)}}^k}}\prt{mL + \frac{240\rho_w^2L^2}{\mu(1 - \rho_w^2)^2}} \frac{\theta^3\sigma^2_*}{{    m^3}\mu^3}\nonumber\\
        &\leq \prt{\frac{K}{t + K}}^{\frac{\theta }{4}} H_0 + \prt{mL + \frac{240\rho_w^2L^2}{\mu(1 - \rho_w^2)^2}} \frac{\theta^3\sigma^2_*}{{    m^3}\mu^3 (t + K)^{\theta  / 4}}\nonumber\\
        &\quad \cdot \sum_{j=0}^{t-1}\frac{( j + K + 1)^{\theta  / 4}m}{(j+K)^3}\label{eq:ds_s1}\\
        &\leq \prt{\frac{K}{t + K}}^{\frac{\theta }{4}} H_0 + \biggl[\prt{mL + \frac{240\rho_w^2L^2}{\mu(1 - \rho_w^2)^2}}\nonumber\\
        &\quad\cdot \frac{{   8}\theta^3 \sigma^2_*}{{    m^2}\mu^3(\theta -8)}\frac{1}{(t+K)^2}\biggr],\label{eq:ds_s2}
    \end{align}\normalsize	
    where \eqref{eq:ds_s1} holds for Lemma \ref{lem:prod}{  by letting $K\geq \frac{\theta}{2m}$} and $\sum_{k=0}^{m - 1}\prt{1 - \frac{\theta}{4{    m}(j + K)}}^k \leq m$. \eqref{eq:ds_s2} holds because{  when $K\geq \frac{\theta}{2}\geq \frac{\theta}{2m}$,
    
    \small 
    \begin{align*}
        \prt{\frac{j + K + 1}{j + K}}^{\frac{\theta}{4}} &\leq \prt{1 + \frac{1}{K}}^{\frac{\theta}{4}}\leq \prt{1 + \frac{2}{\theta}}^{\frac{\theta}{4}}\leq \exp\prt{\frac{1}{2}}\leq 2,
    \end{align*}}\normalsize
    and when $\theta  > 12$,
    \small
    \begin{align*}
        \sum_{j=0}^{t - 1}(j + K)^{\theta /4 - 3} &\leq \int_0^t (x + K)^{\theta / 4 - 3} \mathrm{dx}\leq \frac{4}{\theta  - 8}(t + K)^{\theta  / 4 -2}.
    \end{align*}\normalsize
\end{proof}

\subsection{Proof of Lemma \ref{lem:Atl_ds}}
\label{app:lem_Atl_ds}
\begin{proof}

	{\sp Lemma \ref{lem:At_ds} provides two upper bounds in the form of $H_t\leq \mathcal{H}(\alpha_t)$ for some $\mathcal{H}(\alpha_t)$ depending on the choice of the stepsize policy. Applying the upper bounds to \eqref{eq:Atl} in Lemma \ref{lem:lya} and invoking Lemma \ref{lem:sigma}, we obtain
	\begin{equation}
		\label{eq:Htl_s1}
		\begin{aligned}
			& H_t^{\ell} \leq \prt{1 - \frac{\alpha_t\mu}{4}}^{\ell}\mathcal{H}(\alpha_t) + 2\brk{\frac{\alpha_t^3Lm\sigma^2_*}{4}\prt{1 + \frac{240\alpha_t^2\rho_w^2L^3}{\mu(1-\rho_w^2)^2}}\right.\\
			&\quad \left. + \frac{120\alpha_t^3\rho_w^2 L^2}{\mu (1-\rho_w^2)^2}\sigma_*^2}{  \frac{4}{\alpha_t\mu}}.
		\end{aligned}
	\end{equation}
	}
    % \small
    % \begin{equation}
	% 	\label{eq:Htl_s1}
	% 	\begin{aligned}
	% 	        & H_t^{\ell} \leq \prt{1 - \frac{\alpha_t\mu}{4}}^{\ell}\crk{\prt{\frac{K}{t + K}}^{\frac{\theta }{4}} H_0 + \prt{mL + \frac{240\rho_w^2L^2}{\mu(1 - \rho_w^2)^2}}\right.\\
	% 	        &\left.\quad\cdot \frac{{  8}\theta^3 \sigma^2_*}{{    m^2}\mu^3(\theta -8)}\frac{1}{(t + K)^2}}\\
	% 	        &\quad  + 2\brk{\alpha_t\svar\prt{1 + \frac{240\alpha_t^2\rho_w^2L^3}{\mu(1-\rho_w^2)^2}} + \frac{120\alpha_t^3\rho_w^2 L^2}{\mu (1-\rho_w^2)^2}\sigma_*^2}{  \frac{4}{\alpha_t\mu}}.
	% 	        &\leq \prt{\frac{K}{t + K}}^{\frac{\theta }{4}} H_0 + {  \frac{4\theta^2 L\sigma^2_*}{m^2\mu^3}\prt{m + \frac{240\rho_w^2 L}{\mu(1-\rho_w^2)^2}}\frac{1}{(t + K)^2}}\\
	% 	        &\quad + \prt{mL + \frac{240\rho_w^2L^2}{\mu(1 - \rho_w^2)^2}} \frac{{  8}\theta^3 \sigma^2_*}{{    m^2}\mu^3(\theta -8)}\frac{1}{(t + K)^2},
	% 	    \end{aligned}
	% \end{equation}\normalsize
	
	{\kh 
	If we use diminishing stepsizes $\alpha_t = \frac{\theta}{m\mu(t + K)}$, relation \eqref{eq:Htl_s1} and Lemma \ref{lem:At_ds} yield
	\small 
	\begin{align*}
		H_t^{\ell}&\leq \prt{\frac{K}{t + K}}^{\frac{\theta }{4}} H_0 + {  \frac{4\theta^2 L\sigma^2_*}{m^2\mu^3}\prt{m + \frac{240\rho_w^2 L}{\mu(1-\rho_w^2)^2}}\frac{1}{(t + K)^2}}\\
		&\quad + \prt{mL + \frac{240\rho_w^2L^2}{\mu(1 - \rho_w^2)^2}} \frac{{  8}\theta^3 \sigma^2_*}{{    m^2}\mu^3(\theta -8)}\frac{1}{(t + K)^2}.
	\end{align*}\normalsize

	If we use a constant stepsize $\alpha_t = \alpha$, then \eqref{eq:Htl_s1} and Lemma \ref{lem:sigma} lead to 
	\small
	\begin{align*}
		H_t^{\ell} &\leq \prt{1 - \frac{\alpha\mu}{4}}^{mt} H_0 + \frac{4\alpha^2}{\mu} \prt{mL + \frac{240\rho_w^2L^2}{\mu(1 - \rho_w^2)^2}} \sigma_*^2\\
		&\quad + \frac{4\alpha^2 L}{\mu}\prt{ m + \frac{240\rho_w^2 L}{\mu(1-\rho_w^2)^2}}\sigma^2_*.
	\end{align*}\normalsize
	}
    
    {\sp Rearranging the terms and noting that $\theta > 12$}, we obtain the desired result.
\end{proof}

\subsection{Proof of Lemma \ref{lem:opt1}}
\label{app:lem_opt1}
\begin{proof}
	Apply Lemma \ref{lem:cons1} into Lemma \ref{lem:xbar0} and note $\alpha_t \leq \frac{1}{\mu}$, we have 
	\begin{align*}
		&\E\brk{\norm{\bx{t}{\ell + 1} - \bxs{\ell + 1}}^2}
		\leq (1-\frac{\alpha_t\mu}{2}) \E\brk{\norm{\bx{t}{\ell} - \bxs{\ell}}^2}\\
		&\quad + 2\alpha_t\svar + \frac{2\alpha_t L^2}{n}\prt{\frac{{   1}}{\mu} + \alpha_t}\crk{\prt{\frac{1+\rho_w^2}{2}}^{mt}
		\right.\\
		&\left. \quad \cdot\norm{\x_0^0 - \1(\bar{x}_0^0)^{\T}}^2
		+ \frac{4\hat{X}_1}{(1-\rho_w^2)^2}\alpha_t^2}
	\end{align*}
	
	Invoke relation \eqref{eq:in_out} {    and Lemma \ref{lem:sigma}}, we obtain
	\begin{align*}
		&\E\brk{\norm{\bar{x}_{t + 1}^0 - x^*}^2}
		\leq (1-\frac{\alpha_t\mu}{2})^{m}\E\brk{\norm{\bar{x}_t^0 - x^*}^2}\\
		&+ {  \frac{\alpha_t^3Lm\sigma^2_*}{2}}\brk{\sum_{k=0}^{m-1} \prt{1 - \frac{\alpha_t\mu}{2}}^k} + \frac{{   4}\alpha_tL^2}{n\mu^2}\crk{\prt{\frac{1+\rho_w^2}{2}}^{mt}\right.\\
		&\left. \cdot\norm{\x_0^0 - \1(\bar{x}_0^0)^{\T}}^2 + \frac{4\hat{X}_1}{(1-\rho_w^2)^2}\alpha_t^2}\brk{\sum_{k=0}^{m-1} \prt{1 - \frac{\alpha_t\mu}{2}}^k}
	\end{align*}
	
	Unroll the above, we have 
	\small
	\begin{align*}
		& \E\brk{\norm{\bar{x}_{t}^0 - x^*}^2}
		\leq \prod_{j = 0}^{t - 1} \prt{1 - \frac{\alpha_j\mu}{2}}^m {\norm{\bar{x}_0^0 - x^*}^2}\\
		&+ {  \frac{mL\sigma^2_*}{2}}\sum_{j=0}^{t - 1}\crk{\brk{\prod_{q = j + 1}^{t - 1} \prt{1 - \frac{\alpha_q\mu}{2}}^m} {   \alpha_j^3}\brk{\sum_{k=0}^{m-1} \prt{1 - \frac{\alpha_j\mu}{2}}^k}}\\ 
		&\quad + \sum_{j=0}^{t - 1}\biggr\{\brk{\prod_{q = j + 1}^{t - 1} \prt{1 - \frac{\alpha_q\mu}{2}}^m} \frac{{   4}\alpha_jL^2}{n\mu^2}\brk{\prt{\frac{1+\rho_w^2}{2}}^{mj}\right. \\
		&\left.\quad \cdot\norm{\x_0 - \1\bar{x}_0^{\T}}^2 + \frac{4\hat{X}_1}{(1-\rho_w^2)^2}\alpha_j^2}\brk{\sum_{k=0}^{m-1} \prt{1 - \frac{\alpha_j\mu}{2}}^k}\biggr\}
	\end{align*}\normalsize
	
	Similar to those in deriving Lemma \ref{lem:At_ds} and by $K\geq\theta$, we obtain
	\small
	\begin{align*}
		& \E\brk{\norm{\bar{x}_{t}^0 - x^*}^2} \leq \prt{\frac{K}{t + K}}^{\frac{\theta}{2}}{\norm{\bar{x}_0^0 - x^*}^2}\\
		&\quad + {  \frac{2\theta^3L\sigma^2_*}{m\mu^3(\theta - 4)}\frac{1}{(t + K)^2}} + \frac{{   96} \theta^3 L^2\hat{X}_1}{nm^2\mu^5(1-\rho_w^2)^2(\theta - 4)}\frac{1}{(t + K)^2}\\
		&\quad + \prt{\frac{K}{t + K}}^{\frac{\theta}{2}} \frac{{   96} L^2 }{n\mu^3(1-\rho_w^2)}{\norm{\x_0^0 - \1(\bar{x}_0^0)^{\T}}^2}.
	\end{align*}\normalsize
	
	The last term is because $(t + K)^{\theta /2 - 1}q_0^t$ is decreasing in $t$ with $q_0 := \prt{\frac{1 + \rho_w^2}{2}}^m$, then 
	\begin{align*}
		&\quad \frac{1}{\ln q_0} d\prt{(t + K)^{\frac{\theta }{2} - 1}q_0^t}\\
		&= \frac{1}{\ln q_0} \prt{\frac{\theta  }{2} - 1}\prt{t + K}^{\frac{\theta  }{2} - 2}q_0^t \mathrm{dt} + (t + K)^{\frac{\theta  }{2} -1}q_0^t \mathrm{dt}\\
		&\geq \frac{1}{2}(t + K)^{\frac{\theta  }{2} - 1}q_0^t dt.
	\end{align*}
	
	Thus, 
	\begin{align*}
		& \sum_{j = 0}^{t - 1}(j + K)^{\frac{\theta  }{2} - 1}q_0^j \leq \int_0^{\infty} (t + K)^{\theta /2 - 1}q_0^t \mathrm{dt}\\    
		&\leq \frac{2}{\ln q_0}\int_K^{\infty} \frac{\mathrm{d}\prt{t^{\frac{\theta  }{2} - 1} q_0^{t - K}}}{\mathrm{dt}}  = -\frac{2 K^{\frac{\theta  }{2} - 1}}{\ln q_0}\leq \frac{4 K^{\frac{\theta  }{2} - 1}}{m(1 - \rho_w^2)}.
	\end{align*}
\end{proof}

% \subsection{Proof of Lemma \ref{lem:Fell}}
% \label{app:lem_Fell} 
% \begin{proof}
%      {It holds that} 
%     \begin{align}
%         &\E\brkn{\normn{\nabla \Fp{\ell}(\x_t^{\ell})}^2} \leq 3\E\brkn{\normn{\nabla \Fp{\ell}(\x_t^{\ell}) - \nabla \Fp{\ell}(\1(\bxs{\ell})^{\T})}^2}\nonumber\\
%         & + 3\E\brkn{\normn{\nabla \Fp{\ell}(\1(x^{*})^{\T})}^2}\nonumber\\
%         & + 3\E\brkn{\normn{\nabla \Fp{\ell}(\1(\bxs{\ell})^{\T}) - \nabla \Fp{\ell}(\1(x^{*})^{\T})}}\nonumber\\
%         &\leq 6L^2 n \E\brkn{\normn{\bx{t}{\ell} - \bxs{\ell}}^2} + 6L^2{\sum}_{i=1}^n\E\brkn{\normn{\xitl - \bx{t}{\ell}}^2}\nonumber\\
%         &\quad + 3{\sum}_{i=1}^n \E\brkn{\normn{\nabla \fp{i}{\ell}(x^*)}^2}\nonumber\\
%         &\quad + 3\E\brkn{\normn{\nabla \Fp{\ell}(\1(\bxs{\ell})^{\T}) - \nabla \Fp{\ell}(\1(x^{*})^{\T})}^2}\label{eq:fell1}
%     \end{align}
    
%     We use $\svar$ to bound the last term in \eqref{eq:fell1}. From \eqref{eq:L}: 
%     \small
%     \begin{align*}
%         &\hspace{0.5ex}\E\brkn{\normn{\nabla \Fp{\ell}(\1(\bxs{\ell})^{\T}) - \nabla \Fp{\ell}(\1(x^{*})^{\T})}^2}\\
%         & = \E\brk{\sumn\normn{\nabla \fp{i}{\ell}(\bxs{\ell}) - \nabla \fp{i}{\ell}(x^*)}^2}\\
%         &\leq \E\brk{2L\sumn (\fp{i}{\ell}(\bxs{\ell}) - \fp{i}{\ell}(x^*) - \langle{\nabla \fp{i}{\ell}(x^*), \bxs{\ell} - x^*}\rangle)}\\
%         &= 2nL \E\brkn{D_{\bar{s}_\ell}(\bxs{\ell}, x^*)}
%         % &= 2nL\E\brk{\frac{1}{n}\sumn \fp{i}{\ell}(\bxs{\ell}) - \frac{1}{n}\sumn \fp{i}{\ell}(x^*) - \inpro{\frac{1}{n}\sumn\nabla \fp{i}{\ell}(x^*), \bxs{\ell} - x^*}}\\
%         \leq 2nL\svar.
%     \end{align*}\normalsize
    
%      {Next, we} bound $\sumn \E\brkn{\normn{\nabla \fp{i}{\ell}(x^*)}^2}$ using $\sigma^2_*$: 
%     \begin{align*}
%         \sumn \E\brkn{\normn{\nabla \fp{i}{\ell}(x^*)}^2} &= \sumn\frac{1}{m}\sum_{j=1}^m\norm{\nabla f_{i,j}(x^*)}^2 = n\sigma^2_*.
%     \end{align*}
    
%      {Combining the last} two steps and \eqref{eq:fell1} finishes the proof of Lemma \ref{lem:Fell}. 
%     % \begin{align*}
%         %     \E\brk{\norm{\nabla \Fp{\ell}(\x_t^{\ell})}^2} &\leq 6L^2 n \E\brk{\norm{\bx{t}{\ell} - \bxs{\ell}}^2} + 6L^2\sumn\E\brk{\norm{\xitl - \bx{t}{\ell}}^2}\\
%         %     &\quad + 3n\sigma^2_*  + 6nL\svar
%         % \end{align*}
% \end{proof}

\subsection{Proof of Corollary \ref{cor:scvx_complexity}}
\label{app:cor_scvx_complexity}
\begin{proof}
    {  
    Note for $\alpha$ satisfying \eqref{eq:alphat}, 
    \begin{equation*}
        H_0 \ =\order{\frac{n\norm{\bar{x}_0^0 - x^*}^2 + \norm{\x_0^0 - \1(\bar{x}_0^0)^{\T}}^2}{n}}.
    \end{equation*}
    }
    
    Rearrange the result in {Theorem} \ref{cor:combined1} and notice $(1-x)\leq \exp(-x)$. We obtain 
		\begin{align}
			& \frac{1}{n}\sumn\E\brk{\norm{x_{i,T}^0 - x^*}^2} \leq \exp\prt{-\frac{\alpha\mu m T}{4}} H_0 + \frac{4\alpha^2mL\sigma^2_*}{\mu} \nonumber\\
			&\quad + \frac{4\hat{X}_1}{n(1-\rho_w^2)^2}\alpha^2 + \frac{960\rho_w^2 L^2\sigma^2_*}{\mu^2(1-\rho_w^2)^2}\alpha^2\nonumber\\
			&\quad + \exp\prt{-\frac{1-\rho_w^2}{2}mT}\frac{\norm{\x_0^0 - \1(\bar{x}_0^0)^{\T}}^2}{n}\label{eq:scvx_c}.
		\end{align}
		% where 
		% \begin{align*}
		% 	\hat{X}_1 = \max&\crk{\order{\frac{\norm{\x_0^0 - \1(x^*)^{\T}}^2 + \norm{\x_0^0 - \1(\bar{x}_0^0)^{\T}}^2}{n(1-\rho_w^2)}}, \order{(1-\rho_w^2)^2m^2\sigma^2_*},\right.\\
		% 	&\quad \left. \order{mn\sigma^2_*}, \order{\frac{\sigma^2_*}{(1-\rho_w^2)^2}}}
		% \end{align*}

		Denoting the stepsize satisfying \eqref{eq:alphat} as $\bar{\alpha}$ and 
	    using $\tilde{\cO}(\cdot)$ to hide the logarithm factors, it is sufficient to discuss the following two cases:

		\textbf{Case I:} If $\alpha = \frac{4}{{    L} m T}\log\frac{H_0\mu^2{    m}T^2}{\kappa \sigma^2_*}\leq \bar{\alpha}$, then we substitute such an $\alpha{  \leq \frac{4}{\mu m T}\log\frac{H_0\mu^2{    m}T^2}{\kappa \sigma^2_*}}$ into \eqref{eq:scvx_c} and get
		\begin{align*}
			& \frac{1}{n}\sumn\E\brk{\norm{x_{i,T}^0 - x^*}^2} = \tilde{\cO}\prt{\frac{\kappa \sigma^2_*}{\mu^2 m T^2}}\\
			&\quad + \exp\prt{-\frac{1-\rho_w^2}{2}mT}\frac{\norm{\x_0^0 - \1(\bar{x}_0^0)^{\T}}^2}{n}\\
			&\quad + \tilde{\cO}\prt{\frac{\hat{X}_1}{{    L^2}nm^2(1-\rho_w^2)^2 T^2}} + \tilde{\cO}\prt{\frac{\sigma^2_*}{{   \mu^2}(1-\rho_w^2)^2m^2 T^2}}.
		\end{align*}  

		\textbf{Case II:} If $\bar{\alpha} < \frac{4}{{    L} m T}\log\frac{H_0\mu^2{    m}T^2}{\kappa \sigma^2_*}{  \leq \frac{4}{\mu m T}\log\frac{H_0\mu^2{    m}T^2}{\kappa \sigma^2_*}}$, {  we substitute $\bar\alpha$ into \eqref{eq:scvx_c} and obtain},
		\begin{align*}
			& \frac{1}{n}\sumn\E\brk{\norm{x_{i,T}^0 - x^*}^2} = \exp\prt{-\frac{\bar\alpha\mu m T}{4}} H_0\\
			&\quad + \exp\prt{-\frac{1-\rho_w^2}{2}mT}\frac{\norm{\x_0^0 - \1(\bar{x}_0^0)^{\T}}^2}{n} + \tilde{\cO}\prt{\frac{\kappa\sigma^2_*}{\mu^2mT^2}}  \\
			&\quad + \tilde{\cO}\prt{\frac{\hat{X}_1}{nm^2{    L^2}(1-\rho_w^2)^2T^2}} + \tilde{\cO}\prt{\frac{\sigma^2_*}{(1-\rho_w^2)^2\mu^2m^2T^2}}.
		\end{align*}

		We finish our proof by noting that
		\small
		{  
		\begin{align*}
			\hat{X}_1 = &\order{\frac{\prt{n\norm{\bar{x}_0^0 - x^*}^2 + \norm{\x_0^0 - \1(\bar{x}_0^{0})^{\T}}^2}L^2}{1-\rho_w^2}+ \frac{mn\sigma^2_*}{1-\rho_w^2}}.
		\end{align*}
		}\normalsize

		
		% \begin{align*}
		% 	\frac{1}{n}\sumn\E\brk{\norm{x_{i,T}^0 - x^*}^2} &= \exp\prt{-\frac{\alpha\mu m T}{4}} H_0 + \tilde{\cO}\prt{\frac{\kappa \sigma^2_*}{\mu^2 m T^2}}\\
		% 	&\quad + \tilde{\cO}\prt{\frac{\prt{\norm{\x_0^0 - \1(x^*)^{\T}}^2 + \norm{\x_0^0 - \1(\bar{x}_0^{0})^{\T}}^2}\kappa^2}{(1-\rho_w^2)^3nm^2T^2}}\\
		% 	&\quad + \tilde{\cO}\prt{\frac{\kappa^3\sigma^2_*}{m\mu^2(1-\rho_w^2)^3T^2}} + \exp\prt{-\frac{1-\rho_w^2}{2}mT}\frac{\norm{\x_0^0 - \1(\bar{x}_0^0)^{\T}}^2}{n}\\
		% 	&\quad + \tilde{\cO}\prt{\frac{\kappa^2\sigma^2_*}{(1-\rho_w^2)^2\mu^2m^2T^2}}
		% \end{align*}
\end{proof}


\section{Proofs for the Nonconvex Case}
            {\kh~
            \subsection{Proof of Lemma \ref{as:bounded_var}}
            \label{app:lem_bounded_var}
            \begin{proof}
                The proof is similar to \cite[Proposition 2]{mishchenko2020random}, we present it here for completeness. By Assumption \ref{as:comp_fun}, we have 
                \begin{align*}
                    \norm{\nabla f_{i,\ell}(x)} \leq 2L \prt{f_{i,\ell}(x) - \bar{f}_{i,\ell}}, \ \forall x\in\R^p, \ i,\ell.
                \end{align*}
                Therefore, 
                \begin{align*}
                    &\frac{1}{mn}\sumn\sum_{\ell=1}^m \norm{\nabla f_{i,\ell}(x) - \nabla f(x)}^2
                    \leq \frac{1}{mn}\sumn\sum_{\ell=1}^m\norm{\nabla f_{i,\ell}(x)}^2\\
                    &\leq \frac{2L}{mn}\sumn\sum_{\ell=1}^m\prt{f_{i,\ell}(x) - \bar{f}_{i,\ell}}\\
                    &= 2L(f(x) - \bar{f}) + 2L\prt{\bar{f} - \frac{1}{mn}\sumn\sum_{\ell = 1}^m \bar{f}_{i,\ell}}.
                \end{align*}

                We have $A= 2L > 0$ and $B^2 = 2L\prt{\bar{f} - \frac{1}{mn}\sumn\sum_{\ell = 1}^m \bar{f}_{i,\ell}}\geq 0$.
            \end{proof}
            }
		\subsection{Proof of Lemma \ref{lem:descent-property}}
		\label{app:lem_descent-property}
		
		\begin{proof}
			By $L$-smoothness of the objective function $f$, we obtain
			\begin{equation}\small
				\label{eq:lem-desecent-1}
				\begin{aligned}
					& f(\bx{t+1}{0}) \leq f(\bx{t}{0}) - \inpro{\nabla f(\bx{t}{0}), \bx{t}{0}-\bx{t+1}{0}} + \frac{L}{2}\norm{\bx{t+1}{0}-\bx{t}{0}}^2\\
					&{\kh = f(\bx{t}{0}) - \alpha m \inpro{\nabla f(\bx{t}{0}), \frac{1}{mn} \sum_{\ell=0}^{m-1}\sum_{i=1}^{n} \nabla f_{i,\pi_\ell^i}(x_{i,t}^\ell)}}\\
					&\quad{\kh + \frac{L}{2}\norm{\frac{\alpha}{n} \sum_{\ell=0}^{m-1}\sum_{i=1}^{n} \nabla f_{i,\pi_\ell^i}(x_{i,t}^\ell)}^2}\\
					& = f(\bx{t}{0}) - \frac{\alpha{\kh m}}{2}\norm{\nabla f(\bx{t}{0})}^2\\
					&\quad - \frac{{\kh \alpha m}}{2}\prt{{\kh 1 - \alpha m L}}\norm{{\kh~\frac{1}{mn} \sum_{\ell=0}^{m-1}\sum_{i=1}^{n} \nabla f_{i,\pi_\ell^i}(x_{i,t}^\ell)}}^2 \\
					&\quad + \frac{\alpha {\kh m}}{2}\norm{{\kh~\frac{1}{mn} \sum_{\ell=0}^{m-1}\sum_{i=1}^{n} \nabla f_{i,\pi_\ell^i}(x_{i,t}^\ell)}- \nabla f(\bx{t}{0})}^2,
				\end{aligned}
			\end{equation}\normalsize
			where {\kh we invoke} $\inpro{a,b}=(\norm{a}^2+\norm{b}^2-\norm{a-b}^2)/2$. 
			%upon setting $a=\sqrt{\alpha}\nabla f(\bx{t}{0})$ and $b=\frac{1}{\sqrt{\alpha}}(\bx{t}{0} - \bx{t+1}{0})$.
			
			% Note that the third term in \eqref{eq:lem-desecent-1} can be removed since $\alpha$ is chosen smaller than $1/L$. Hence, the last term is the only one to be estimated in \eqref{eq:lem-desecent-1}. 
			% We first expand $\bx{t}{0}-\bx{t+1}{0}$ and $\nabla f(\bx{t}{0})$ as
			% \begin{equation}
			% 	\label{eq:lem-desecent-2}
			% 	\begin{aligned}
			% 		\bx{t}{0}-\bx{t+1}{0}&=\frac{\alpha}{n} \sum_{\ell=0}^{m-1}\sum_{i=1}^{n} \nabla f_{i,\pi_\ell^i(x_{i,t}^\ell)},\\
			% 		\nabla f(\bx{t}{0}) &= \frac{1}{n}\sum_{i=1}^{n}\prt{\frac{1}{m}\sum_{\ell=1}^{m}\nabla f_{i,\ell}(\bx{t}{0})}\\
			% 		& = \frac{1}{mn}\sum_{\ell=0}^{m-1}\sum_{i=1}^{n}\nabla f_{i,\pi_\ell^i}(\bx{t}{0}).
			% 	\end{aligned}
			% \end{equation}

			Then, utilizing $L$-smoothness of each component function yields
			% \begin{equation}
			% 	\label{eq:lem-desecent-3}
			% 	\begin{aligned}
			% 		&\quad \norm{\frac{\bx{t}{0}-\bx{t+1}{0}}{\alpha}- \nabla f(\bx{t}{0})} \\
			% 		&\leq \frac{1}{mn} \sum_{\ell=0}^{m-1}\sum_{i=1}^{n}\|\nabla f_{i,\pi_\ell^i(x_{i,t}^\ell)}- \nabla f_{i,\pi_\ell^i}(\bx{t}{0})\| \\
			% 		&\leq \frac{L}{mn} \sum_{\ell=0}^{m-1}\sum_{i=1}^{n}\|x_{i,t}^\ell-  \bx{t}{0}\| \\
			% 		&\leq \frac{L}{mn} \sum_{\ell=0}^{m-1}\sum_{i=1}^{n}\|x_{i,t}^\ell-  \bx{t}{\ell}\| + \frac{L}{m} \sum_{\ell=0}^{m-1}\norm{\bx{t}{\ell}-\bx{t}{0}}.
			% 	\end{aligned}
			% \end{equation}
			% Taking square on both sides of \eqref{eq:lem-desecent-3} yields
			\begin{equation}
				\label{eq:lem-desecent-4}
				\begin{aligned}
					&{\kh~\norm{\frac{1}{mn} \sum_{\ell=0}^{m-1}\sum_{i=1}^{n} \nabla f_{i,\pi_\ell^i}(x_{i,t}^\ell)- \nabla f(\bx{t}{0})}^2}\\
					&\leq \frac{L^2}{mn}\sum_{\ell = 0}^{m-1}\sum_{i=1}^n \norm{x_{i,t}^{\ell} - \bx{t}{0}}^2\\
					& \leq \frac{2L^2}{mn} \sum_{\ell=0}^{m-1}\norm{\x_t^\ell-  \1(\bx{t}{\ell})^\T}^2 + \frac{2L^2}{m} \sum_{\ell=0}^{m-1}\norm{\bx{t}{\ell}-\bx{t}{0}}^2.
				\end{aligned}
			\end{equation}	

			Inserting \eqref{eq:lem-desecent-4} into \eqref{eq:lem-desecent-1} and using the condition $\alpha\leq \frac{1}{mL}$ finish the proof. 
		\end{proof}
		
		\subsection{Proof of Lemma \ref{lem:noncvx-con-err}}
		\label{app:lem_noncvx-con-err}
		%%% proof under bounded variance assumption
		{\kh~
		\begin{proof}
			By the update \eqref{eq:comp} and Young's inequality for $q = \frac{1 + \rho_w^2}{2\rho_w^2}$, we have 
			\small
			\begin{equation}
				\label{eq:noncvx-lem-1}
				\begin{aligned}
					&\norm{\x_t^{\ell + 1} - \1(\bx{t}{\ell + 1})^{\T}}^2 \leq \norm{\prt{W - \frac{\1\1^{\T}}{n}}\prt{\x_t^{\ell} - \alpha \nabla \Fp{\ell}(\x_t^{\ell})}}^2\\
					&\leq \frac{1 + \rho_w^2}{2}\norm{\x_t^{\ell} - \1(\bx{t}{\ell})^{\T}}^2 + \frac{2\alpha^2}{1-\rho_w^2}\norm{\nabla \Fp{\ell}(\x_t^{\ell})}^2.
 				\end{aligned}
			\end{equation}\normalsize

			{\sp It follows that}
			\begin{equation}
				\label{eq:noncvx-lem-2}
				\begin{aligned}
					& \sum_{\ell = 0}^{m-1} \norm{\x_t^{\ell} - \1(\bx{t}{\ell})^{\T}}^2 \leq \frac{2}{1-\rho_w^2} \norm{\x_t^0 - \1(\bx{t}{0})^{\T}}^2\\
					&\quad +  \frac{2\alpha^2}{1-\rho_w^2}\sum_{\ell = 0}^{m-1}\sum_{j=0}^{\ell - 1}\prt{\frac{1 + \rho_w^2}{2}}^{\ell - j - 1}\sum_{i=1}^n\norm{\nabla \fp{i}{j}(x_{i,t}^j)}^2.
				\end{aligned}
			\end{equation}

			Next consider the last term in \eqref{eq:noncvx-lem-2}. We have 
			\small
			\begin{align}
				&\frac{1}{3}\sum_{\ell = 0}^{m-1}\sum_{j=0}^{\ell - 1}\prt{\frac{1 + \rho_w^2}{2}}^{\ell - j - 1}\sum_{i=1}^n\norm{\nabla \fp{i}{j}(x_{i,t}^j)}^2\nonumber\\
				&\leq \sum_{\ell = 0}^{m-1}\sum_{j=0}^{\ell - 1}\prt{\frac{1 + \rho_w^2}{2}}^{\ell - j - 1}\sum_{i=1}^n\crk{\norm{\nabla \fp{i}{j}(x_{i,t}^j) - \nabla \fp{i}{j}(\bx{t}{0})}^2\right.\nonumber\\
				&\quad\left.  + \norm{\nabla \fp{i}{j}(\bx{t}{0}) - \nabla f(\bx{t}{0})}^2 + \norm{\nabla f(\bx{t}{0})}^2}\nonumber\\
				&\leq \sum_{\ell = 0}^{m-1}\sum_{j=0}^{\ell - 1}\prt{\frac{1 + \rho_w^2}{2}}^{\ell - j - 1}\sum_{i=1}^n\crk{L^2\norm{x_{i,t}^j - \bx{t}{0}}^2\right.\nonumber\\
				&\quad\left. + \norm{\nabla \fp{i}{j}(\bx{t}{0}) - \nabla f(\bx{t}{0})}^2 + \norm{\nabla f(\bx{t}{0})}^2}\label{eq:noncvx-cons-s1}\\
				&\leq \frac{2L^2}{1-\rho_w^2}\sum_{\ell=0}^{m-1}\sum_{i=1}^n\norm{x_{i,t}^{\ell} - \bx{t}{0}}^2 + \frac{2mn}{1-\rho_w^2}\norm{\nabla f(\bx{t}{0})}^2\nonumber\\
				&\quad + \frac{2m^2n}{1-\rho_w^2}\brk{2A\prt{f(\bx{t}{0}) - \bar{f}} + B^2},\label{eq:noncvx-cons-s2}
			\end{align}\normalsize
			where \eqref{eq:noncvx-cons-s1} comes from Assumption \ref{as:comp_fun}, and \eqref{eq:noncvx-cons-s2} holds by Lemma \ref{as:bounded_var}. Combining \eqref{eq:lem-desecent-4}, \eqref{eq:noncvx-lem-2} and \eqref{eq:noncvx-cons-s2} leads to
			\small
			\begin{equation}
				\label{eq:noncvx-cons-ell}
				\begin{aligned}
					&\sum_{\ell=0}^{m-1}\norm{\x_t^{\ell} - \1(\bx{t}{\ell})^{\T}}^2\leq \frac{2}{1-\rho_w^2}\norm{\x_t^0 - \1(\bx{t}{0})^{\T}}^2 + \frac{12B^2\alpha^2 m^2n}{(1-\rho_w^2)^2}\nonumber\\
					&\quad + \frac{12mn\alpha^2}{(1-\rho_w^2)^2}\norm{\nabla f(\bx{t}{0})}^2 + \frac{24\alpha^2nL^2}{(1-\rho_w^2)^2}\sum_{\ell = 0}^{m-1}\norm{\bx{t}{\ell} - \bx{t}{0}}^2\nonumber\\
					&\quad + \frac{24\alpha^2 L^2}{(1-\rho_w^2)^2}\sum_{\ell = 0}^{m-1}\norm{\x_t^\ell - \1(\bx{t}{\ell})^{\T}}^2\\
					&\quad + \frac{24 A\alpha^2 m^2n}{(1-\rho_w^2)^2}\prt{f(\bx{t}{0}) - \bar{f}}.
				\end{aligned}
			\end{equation}\normalsize

			Similar to \eqref{eq:noncvx-cons-s2}, we have 
			\small
			\begin{equation}
				\label{eq:noncvx-cons-bar}
				\begin{aligned}
					&\sum_{\ell = 0}^{m-1}\norm{\bx{t}{\ell} - \bx{t}{0}}^2 = m^2 \alpha^2 \sum_{\ell = 0}^{m-1}\norm{\frac{1}{mn}\sum_{j=0}^{\ell - 1}\sum_{i=1}^n\nabla \fp{i}{j}(x_{i,t}^j)}^2\\
					&\leq \frac{m\alpha^2}{n}\sum_{\ell = 0}^{m-1}\sum_{j=0}^{\ell-1}\sum_{i=1}^n \norm{\nabla \fp{i}{j}(x_{i,t}^j)}^2\\
					&\leq \frac{6m^2\alpha^2L^2}{n}\sum_{\ell=0}^{m-1}\norm{\x_t^\ell - \1(\bx{t}{\ell})^{\T}}^2 + 6m^2\alpha^2L^2\sum_{\ell=0}^{m-1}\norm{\bx{t}{\ell} - \bx{t}{0}}^2\\
					&\quad + 3m^3\alpha^2\brk{2A\prt{f(\bx{t}{0}) - \bar{f}} + B^2} + 3m^3\alpha^2\norm{\nabla f(\bx{t}{0})}^2.
				\end{aligned}
			\end{equation}\normalsize
			
			 {\sp Since $\cL_t=\frac{1}{n}\sum_{\ell=0}^{m-1}\norm{\x_t^{\ell} - \1(\bx{t}{\ell})^{\T}}^2 + \sum_{\ell = 0}^{m-1}\norm{\bx{t}{\ell} - \bx{t}{0}}^2$}, we have 
			\small
			\begin{align*}
				&\prt{1 - 6m^2\alpha^2L^2 - \frac{24\alpha^2L^2}{(1-\rho_w^2)^2}}\cL_t \leq \frac{2}{n(1-\rho_w^2)}\norm{\x_t^0 - \1(\bx{t}{0})^{\T}}^2\\
				&\quad + \frac{3m^2\alpha^2B^2(m + 4)}{(1-\rho_w^2)^2} + \frac{3\alpha^2m(4 + m^2)}{(1-\rho_w^2)^2}\norm{\nabla f(\bx{t}{0})}^2\\
				&\quad + \frac{6m^2\alpha^2 A(4 + m)}{(1-\rho_w^2)}\prt{f(\bx{t}{0})  - \bar{f}}.
			\end{align*}\normalsize
			
			Let 
			\begin{equation*}
				\alpha\leq \min\crk{\frac{1}{2\sqrt{6}mL}, \frac{1-\rho_w^2}{4\sqrt{6}L}}.
			\end{equation*}
			We obtain the desired result for $\cL^t$. {\sp Then}, from \eqref{eq:noncvx-lem-1}, we have 
			\small
			\begin{equation}
				\label{eq:noncvx-cons-s3}
				\begin{aligned}
					&\norm{\x_{t+1}^0 - \1(\bx{t+1}{0})^{\T}}^2 = \norm{\x_{t}^m - \1(\bx{t}{m})^{\T}}^2\\
					&\leq \prt{\frac{1 + \rho_w^2}{2}}^m\norm{\x_t^0 - \1(\bx{t}{0})^{\T}}^2\\
					&\quad + \frac{2\alpha^2}{1-\rho_w^2}\sum_{j=0}^{m-1}\prt{\frac{1 + \rho_w^2}{2}}^{m-j-1}\norm{\nabla \Fp{j}(\x_t^j)}^2\\
					&\leq \prt{\frac{1 + \rho_w^2}{2}}^m\norm{\x_t^0 - \1(\bx{t}{0})^{\T}}^2 + \frac{2\alpha^2}{1-\rho_w^2}\sum_{j=0}^{m-1}\norm{\nabla \Fp{j}(\x_t^j)}^2\\
					&\leq \prt{\frac{1 + \rho_w^2}{2}}^m\norm{\x_t^0 - \1(\bx{t}{0})^{\T}}^2 + \frac{12\alpha^2 L^2}{1-\rho_w^2}\sum_{j = 0}^{m-1}\norm{\x_t^{j} - \1(\bx{t}{j})^{\T}}^2\\
					&\quad + \frac{12\alpha^2 L^2n}{1-\rho_w^2}\sum_{j=0}^{m-1}\norm{\bx{t}{j}-\bx{t}{0}}^2 +  \frac{6\alpha^2mn}{1-\rho_w^2}\norm{\nabla f(\bx{t}{0})}^2\\
					&\quad + \frac{6\alpha^2mn}{1-\rho_w^2}\brk{2A\prt{f(\bx{t}{0}) - \bar{f}} + B^2}.
				\end{aligned}
			\end{equation}\normalsize

			
		\end{proof}}

	{\kh~
	\subsection{Proof of Lemma \ref{lem:Qt}}
	\label{app:lem_Qt}
	\begin{proof}
		Substituting $\cL_t$ into Lemma \ref{lem:descent-property} yields
		\begin{equation}
			\label{eq:ncvx_descent_new}
			\begin{aligned}
				&f(\bx{t + 1}{0})\leq f(\bx{t}{0}) - \frac{m\alpha}{2}\norm{\nabla f(\bx{t}{0})}^2 + \alpha L^2\cL_t\\
				&\leq f(\bx{t}{0}) - \frac{m\alpha}{2}\norm{\nabla f(\bx{t}{0})}^2 + \frac{4\alpha L^2}{n(1-\rho_w^2)}\norm{\x_t^0 - \1(\bx{t}{0})^{\T}}^2\\
				&\quad + \frac{6m^2\alpha^3B^2(m + 4)L^2}{(1-\rho_w^2)^2} + \frac{6\alpha^3m(4 + m^2)L^2}{(1-\rho_w^2)^2}\norm{\nabla f(\bx{t}{0})}^2\\
				&\quad + \frac{12m^2\alpha^3L^2 A(4 + m)}{(1-\rho_w^2)}\prt{f(\bx{t}{0})  - \bar{f}}.
			\end{aligned}
		\end{equation}

		Combining the two recursions in Lemma \ref{lem:noncvx-con-err} and letting $\alpha \leq \prt{\frac{(1-\rho_w^2)^3}{192L^2}}^{1/2}$, we have 
		\begin{equation}
			\label{eq:ncvx_cons_t}
			\begin{aligned}
				&\norm{\x_{t+1}^0 - \1(\bx{t+1}{0})^{\T}}^2 \leq \frac{3 + \rho_w^2}{4}\norm{\x_t^0 - \1(\bx{t}{0})^{\T}}^2\\
				&\quad +  \frac{6\alpha^2mn B^2}{1-\rho_w^2}\prt{1 + \frac{12\alpha^2L^2 m(m + 4)}{(1-\rho_w^2)^2}}\\
				&\quad  +  \frac{6\alpha^2mn}{1-\rho_w^2}\prt{1 + \frac{12\alpha^2 L^2(m^2 + 4)}{(1-\rho_w^2)^2}}\norm{\nabla f(\bx{t}{0})}^2\\
				&\quad + \frac{12A\alpha^2mn}{1-\rho_w^2}\prt{1 + \frac{12\alpha^2L^2 m(m+4)}{(1-\rho_w^2)^2}}\prt{f(\bx{t}{0}) - \bar{f}}\\
				&\leq  \frac{3 + \rho_w^2}{4}\norm{\x_t^0 - \1(\bx{t}{0})^{\T}}^2 +  \frac{12\alpha^2mn B^2}{1-\rho_w^2}\\
				&\quad  +  \frac{12\alpha^2mn}{1-\rho_w^2}\norm{\nabla f(\bx{t}{0})}^2 + \frac{24A\alpha^2mn}{1-\rho_w^2}\prt{f(\bx{t}{0}) - \bar{f}},
			\end{aligned}
		\end{equation}
		where the last inequality holds by letting $\alpha\leq \frac{1-\rho_w^2}{2\sqrt{3}(m + 2)L}$. Combining \eqref{eq:ncvx_descent_new} and \eqref{eq:ncvx_cons_t} yields
		\begin{equation}\small 
			\label{eq:ncvx_fcons}
			\begin{aligned}
				&f(\bx{t + 1}{0}) - \bar{f} + \frac{16\alpha L^2}{n(1-\rho_w^2)^2}\norm{\x_{t + 1}^0 - \1(\bx{t + 1}{0})^{\T}}^2\\
				&\leq \brk{1 + \frac{12m^2\alpha^3L^2 A(4 + m)}{(1-\rho_w^2)} + \frac{384A\alpha^3L^2m}{(1-\rho_w^2)^3}}\prt{f(\bx{t}{0}) - \bar{f}}\\
				&\quad + \frac{16\alpha L^2}{n(1-\rho_w^2)^2}\norm{\x_{t}^0 - \1(\bx{t}{0})^{\T}}^2 + \frac{6m\alpha^3 L^2B^2[m(m + 4) + 32]}{(1-\rho_w^2)^3}\\
				&\quad - \frac{m\alpha}{2}\prt{1 - \frac{12\alpha^2(4 + m^2)L^2}{(1-\rho_w^2)^2} - \frac{384\alpha^2L^2}{(1-\rho_w^2)^3}}\norm{\nabla f(\bx{t}{0})}^2.
			\end{aligned}
		\end{equation}\normalsize

		{\sp Since $Q_t$ is defined as}
		\begin{align*}
			Q_t := f(\bx{t}{0}) - \bar{f} + \frac{16\alpha L^2}{n(1-\rho_w^2)^2}\norm{\x_{t}^0 - \1(\bx{t}{0})^{\T}}^2,
		\end{align*}
		relation \eqref{eq:ncvx_fcons} becomes 
		\begin{equation}\small 
			\label{eq:ncvx_fcons1}
			\begin{aligned}
				&Q_{t + 1} \leq \brk{1 + \frac{12m^2\alpha^3L^2 A(4 + m)}{(1-\rho_w^2)} + \frac{384A\alpha^3L^2m}{(1-\rho_w^2)^3}} Q_t \\
				&\quad - \frac{m\alpha}{4}\norm{\nabla f(\bx{t}{0})}^2 + \frac{6m\alpha^3 L^2B^2[m(m + 4) + 32]}{(1-\rho_w^2)^3},
			\end{aligned}
		\end{equation}
		where we invoke $\alpha\leq \min\crk{\frac{1-\rho_w^2}{4\sqrt{3}L(m+2)}, \frac{(1-\rho_w^2)^{3/2}}{16\sqrt{6}L}}$.
		%Take the sum of \eqref{eq:ncvx_descent_new} and \eqref{eq:ncvx_cons_t}, we have 
		% \small
		% \begin{align*}
		% 	&\sum_{t=0}^{T-1}\prt{f(\bx{t}{0}) - \bar{f}} \leq \brk{1 + \frac{6m^2\alpha^3L^2A(4 + m)}{1-\rho_w^2}}\sum_{t=0}^{T - 1}\prt{f(\bx{t}{0}) -\bar{f}}\\
		% 	&\quad - \frac{m\alpha}{2}\prt{1 - \frac{6\alpha^2 (m^2 + 4)L^2}{(1-\rho_w^2)^2}}\sum_{t=0}^{T-1}\norm{\nabla f(\bx{t}{0})}^2\\
		% 	&\quad + \frac{3m^2\alpha^3B^2(m + 4)L^2 T }{(1-\rho_w^2)^2} + \frac{2\alpha L^2}{n(1-\rho_w^2)}\sum_{t=0}^{T-1}\norm{\x_t^0 - \1(\bx{t}{0})^{\T}}^2,
		% \end{align*}\normalsize
		% and 
		% \small
		% \begin{align*}
		% 	&\sum_{t=0}^{T-1}\norm{\x_t^0 - \1(\bx{t}{0})^{\T}}^2 \leq \frac{4\norm{\x_0^0-\1(\bx{0}{0})^{\T}}^2}{1-\rho_w^2} + \frac{48\alpha^2 mnB^2 T}{(1-\rho_w^2)^2}\\
		% 	&\quad + \frac{48\alpha^2 mn}{(1-\rho_w^2)^2}\sum_{t=0}^{T-1}\norm{\nabla f(\bx{t}{0})}^2 + \frac{96A\alpha^2 mn}{(1-\rho_w^2)^2}\sum_{t=0}^{T-1}\prt{f(\bx{t}{0})-\bar{f}}.
		% \end{align*}\normalsize

		% Combining the above two summations yields
		% \begin{equation}\small
		% 	\label{eq:ncvx_sum}
		% 	\begin{aligned}
		% 		&\sum_{t=0}^{T-1}\prt{f(\bx{t}{0}) - \bar{f}}\\
		% 		&\leq \brk{1 + \frac{6m^2\alpha^3L^2A(4 + m)}{1-\rho_w^2} + \frac{192\alpha^3L^2Am}{(1-\rho_w^2)^3}}\sum_{t=0}^{T - 1}\prt{f(\bx{t}{0}) -\bar{f}}\\
		% 		&\quad - \frac{m\alpha}{2}\prt{1 - \frac{6\alpha^2 (m^2 + 4)L^2}{(1-\rho_w^2)^2} - \frac{192\alpha^2 L^2}{(1-\rho_w^2)^3}}\sum_{t=0}^{T-1}\norm{\nabla f(\bx{t}{0})}^2 \\
		% 		&\quad + \frac{3m\alpha^3B^2L^2 T [m(m + 4) + 32]}{(1-\rho_w^2)^3} +\frac{8\alpha L^2\norm{\x_0^0-\1(\bx{0}{0})^{\T}}^2}{n(1-\rho_w^2)^2}
		% 	\end{aligned}
		% \end{equation}\normalsize

		
	\end{proof}
	}

	

		% \begin{proof}
		% 	According to the update steps in Algorithm \ref{alg:DGD-RR} and recursion \eqref{eq:RR_avg}, the following estimate holds for all $t\geq 1$ and $\ell\geq1$, 
		% 	\small
		% 	\begin{equation}
		% 		\label{eq:noncvx-lem-1}
		% 		\begin{aligned}
		% 			&\quad \norm{\x_t^\ell - \1 (\bx{t}{\ell})^\T} \leq \norm{\prt{W-\frac{1}{n}\1\1^\T}\prt{\x_t^{\ell-1}-\frac{\alpha}{m} \nabla F_{\pi_\ell}(\x_t^{\ell-1}) } }	\\
		% 			&\leq \norm{W^{\ell-1}-\frac{1}{n}\1\1^\T} \norm{\x_t^0 - \1(\bx{t}{0})^\T}\\
		% 			&\quad + \frac{\alpha}{m} \sum_{j=0}^{\ell-1} \norm{W^{\ell-1-j}-\frac{1}{n}\1\1^\T}\norm{\nabla F_{\pi_j}(\x_t^j)}\\
		% 			&\leq \rho_w^{\ell-1}  \norm{\x_t^0 - \1 (\bx{t}{0})^\T} + \frac{\alpha \sqrt{n} G}{m}  \sum_{j=0}^{\ell-1} \rho_w^{\ell-1-j}\\
		% 			& \leq 
		% 			\rho_w^{\ell-1}\norm{\x_t^0 - \1 (\bx{t}{0})^\T} +  \frac{\sqrt{n}G\alpha}{m(1-\rho_w)},
		% 		\end{aligned}
		% 	\end{equation}\normalsize
		% 	where we use the bounded gradient condition in Assumption \ref{as:comp_fun}. Then, by utilizing inequality $(a+b)^2\leq 2(a^2+b^2)$ and the estimate \eqref{eq:noncvx-lem-1}, we obtain
		% 	\begin{equation}
		% 		\label{eq:noncvx-lem-2}
		% 		\begin{aligned}
		% 			& \sum_{\ell=0}^{m-1}\norm{\x_t^\ell-  \1(\bx{t}{\ell})^\T}^2 \leq  \prt{1+2\sum_{\ell=1}^{m-1} \rho_w^{2(\ell-1)}} \norm{\x_t^0 - \1 (\bx{t}{0})^\T}^2\\
		% 			&\quad + \frac{2nG^2\alpha^2}{m(1-\rho_w)^2}\\
		% 			&\leq \frac{3-\rho_w^2}{1-\rho_w^2}\norm{\x_t^0 - \1 (\bx{t}{0})^\T}^2 +  \frac{2nG^2\alpha^2}{m(1-\rho_w)^2}.
		% 		\end{aligned}
		% 	\end{equation}
			

		% 	\begin{comment}
		% 	Let us notice that if $m=1$, Algorithm \ref{alg:DGD-RR} reduces to decentralized gradient descent method (DGD) which has already been extensively studied in both convex and nonconvex setting, see, e.g., \cite{yuan2016convergence,zeng2018nonconvex}. 
		% 	Trivially, when $m=1$, we obtain the following estimate by invoking the estimate \eqref{eq:noncvx-lem-1}
		% 	\begin{align*}
		% 		&\quad\sum_{\ell=0}^{m-1}\norm{\x_t^\ell-  \1(\bx{t}{\ell})^\T}^2 = \norm{\x_t^0-  \1(\bx{t}{0})^\T}^2 = \norm{\x_{t-1}^1-  \1(\bx{t-1}{1})^\T}^2 \\
		% 		&\leq \prt{\norm{\x_{t-1}^0-  \1(\bx{t-1}{0})^\T}+\frac{\sqrt{n}G\alpha}{m}}^2=\prt{\rho_w\norm{\x_{t-1}^0}+\frac{\sqrt{n}G\alpha}{m}}^2\leq \rho_w\norm{\x_{t-1}^0}^2 + \frac{nG^2\alpha^2}{m^2(1-\rho_w)}\\
		% 		&\leq \rho_w^t\norm{\x_0^0}^2 + \frac{nG^2\alpha^2}{m^2(1-\rho_w)}\prt{\sum_{k=0}^{t-1}\rho_w^k} \leq \rho_w^t\norm{\x_0^0}^2+ \frac{nG^2\alpha^2}{m^2(1-\rho_w)^2}\leq D_1 \rho_w^t + \frac{D_2}{m^2}\alpha^2,
		% 	\end{align*}
		% 	where the second line is due to Young's inequality $2\inpro{\sqrt{\varepsilon}a,b/\sqrt{\varepsilon}} \leq \varepsilon a^2 + b^2/\varepsilon$ with $a=\rho_w\norm{\x_{t-1}^0},b=\sqrt{n}G\alpha/m$ and $\varepsilon=\rho_w^{-1}-1$. 
		% 	\end{comment}

		% 	%Next, we turn our attention to the case when $m\geq 2$, and 
		% 	It immediately follows from the estimate \eqref{eq:noncvx-lem-1} that $\norm{\x_{t-1}^m - \1 (\bx{t-1}{m})^\T}\leq \rho_w\norm{\x_{t-1}^0 - \1 (\bx{t-1}{0})^\T} +  \frac{\sqrt{n}G\alpha}{m(1-\rho_w)}$ for all $t\geq1$. 
		% 	Applying Young's inequality, $2\inpro{\sqrt{\varepsilon}a,b/\sqrt{\varepsilon}} \leq \varepsilon a^2 + b^2/\varepsilon\  \forall a,b\geq0,\varepsilon>0$, upon setting $a=\rho_w\norm{\x_{t-1}^0 - \1 (\bx{t-1}{0})^\T},b=\frac{\sqrt{n}G\alpha}{m(1-\rho_w)}$ and $\varepsilon=\rho_w^{-1}-1$, this yields
		% 	\begin{equation}
		% 		\label{eq:noncvx-lem-3}
		% 		\begin{aligned}
		% 			& \norm{\x_t^0 - \1 (\bx{t}{0})^\T}^2 = \norm{\x_{t-1}^m - \1 (\bx{t-1}{m})^\T}^2\\
		% 			& \leq \rho_w\norm{\x_{t-1}^0- \1 (\bx{t-1}{0})^\T}^2 + \frac{nG^2\alpha^2}{m^2(1-\rho_w)^3}\\
		% 			&\leq \rho_w^t\norm{\x_0^0-\1(\bx{0}{0})^\T}^2+\frac{nG^2\alpha^2}{m^2(1-\rho_w)^3}\sum_{k=0}^{t-1}\rho_w^k\\
		% 			& \leq \rho_w^t\norm{\x_0^0}^2+\frac{nG^2\alpha^2}{m^2(1-\rho_w)^4}.
		% 		\end{aligned}
		% 	\end{equation}

		% 	We finalize the proof by merging \eqref{eq:noncvx-lem-2} with \eqref{eq:noncvx-lem-3}.
		% \end{proof}
